Robust Dynamic Resource Allocation via Probabilistic Task Pruning in Heterogeneous Computing Systems

In heterogeneous distributed computing (HC) systems, diversity can exist in both computational resources and arriving tasks. In an inconsistently heterogeneous computing system, task types have different execution times on heterogeneous machines. A method is required to map arriving tasks to machines based on machine availability and performance, maximizing the number of tasks meeting deadlines (defined as robustness). For tasks with hard deadlines (eg those in live video streaming), tasks that miss their deadlines are dropped. The problem investigated in this research is maximizing the robustness of an oversubscribed HC system. A way to maximize this robustness is to prune (ie defer or drop) tasks with low probability of meeting their deadlines to increase the probability of other tasks meeting their deadlines. In this paper, we first provide a mathematical model to estimate a task's probability of meeting its deadline in the presence of task dropping. We then investigate methods for engaging probabilistic dropping and we find thresholds for dropping and deferring. Next, we develop a pruning-aware mapping heuristic and extend it to engender fairness across various task types. We show the cost benefit of using probabilistic pruning in an HC system. Simulation results, harnessing a selection of mapping heuristics, show efficacy of the pruning mechanism in improving robustness (on average by 25%) and cost in an oversubscribed HC system by up to 40%.

==> Sources/heuristics.tex <==


\begin{comment}
\subsection{MinCompletion-MinCompletion (MM)}
This heuristic has seen much use and examination in the literature~\cite{he2003qos,pedemonte2016accelerating,ezzatti2013efficient, salehi2016stochastic}. The PET matrix is used to calculate expected completion times. In the first phase of this two-stage heuristic, the virtual queue is traversed, and for each task in that queue, the machine with the minimum expected completion time is found, and a pair is made. In the second phase, for each machine with a slot in its machine queue, the provisional mapping pairs are examined to find the machine-task pair with the minimum completion time, and the assignment is made to the virtual machine queues. The process repeats itself until all virtual machine queues are full, or until the temporary batch queue is exhausted.

\subsection{MinCompletion-Soonest Deadline (MSD)}
Phase one is as in MM. Phase two selects the tasks for each machine with the soonest deadline. In the event of a tie, the task with the minimum expected completion time is selected, and the overall soonest deadline is chosen. As with MM, after each machine with an available virtual queue slot receives a task from the provisional mapping in phase two, the process is repeated until either the virtual machine queues are full, or the temporary unmapped task queue is empty.

\subsection{MinCompletion-MaxUrgency (MMU)}
Phase two of MMU is focused on urgency. Urgency for task $i$ on machine $j$ is defined as the inverse of the difference between the task deadline ($\delta_i$) and the expected completion time of the task on machine $j$ ($\mathbf{E}[C(t_{ij})]$). Equation~\ref{eq:urg} formally shows the urgency definition.

\begin{equation}\label{eq:urg}
    U_{ij} = \frac{1}{\delta_i-\mathbf{E}[C(t_{ij})]}
\end{equation}

Phase one is the same as the previous heuristics. Using the urgency equation, phase two selects the task-machine pair that has the greatest urgency, and adds that mapping to the virtual queue. The process is repeated until either the temporary batch queue is empty, or until the virtual machine queues are full.

\subsection{Max Ontime Completions (MOC)}
The MOC heuristic is based on an algorithm proposed in \cite{salehi2016stochastic} and uses the PET matrix to calculate completion times. It is also a two-phase heuristic, with a culling step in between, based on finding the robustness of task-machine mappings. The first mapping phase finds, for each task, the machine offering the highest robustness value. The culling phase clears the virtual queue of any tasks that fail to meet a given robustness threshold \(\alpha\). Herein, \(\alpha\) is set to 30\%. This contrasts with PAM, which defers tasks which do not meet the robustness threshold used by the system to drop tasks. The last phase finds the three virtual mappings with the highest robustness and permutes them to find the task-machine pair that maximizes the overall robustness and maps it to that machine's virtual queue. PAM, in contrast, chooses the pair with the minimum completion time. The process repeats until either all tasks in the temporary batch queue are mapped or dropped, or until the virtual machine queues are full. 
\end{comment}

